Toward Stronger Textual Attack Detectors

The landscape of available textual adversarial attacks keeps growing, posing severe threats and raising concerns regarding the deep NLP system's integrity. However, the crucial problem of defending against malicious attacks has only drawn the attention of the NLP community. The latter is nonetheless instrumental in developing robust and trustworthy systems. This paper makes two important contributions in this line of search: (i) we introduce LAROUSSE, a new framework to detect textual adversarial attacks and (ii) we introduce STAKEOUT, a new benchmark composed of nine popular attack methods, three datasets, and two pre-trained models. LAROUSSE is ready-to-use in production as it is unsupervised, hyperparameter-free, and non-differentiable, protecting it against gradient-based methods. Our new benchmark STAKEOUT allows for a robust evaluation framework: we conduct extensive numerical experiments which demonstrate that LAROUSSE outperforms previous methods, and which allows to identify interesting factors of detection rate variations.

==> back.tex <==
\iffalse
\vspace{1cm}

\hline

%They can be divided into two subgroups. Robust training \cite{yoo-qi-2021-towards-improving,zhou2021defense,pruthi-etal-2019-combating} rely on custom training techniques that supposedly allow to anticipate for adversarial attacks. In contrast, detection techniques do not retrain models but rather introduce methods that aim to correctly discriminate between regular inputs and attacks. In our view, the latter are more relevant to real-life scenarios where retraining a model is expansive and cannot anticipate for all upcoming types of attacks. 

%There are only a few works that rely on detection techniques to discriminate attacks from regular inputs in NLP. 

Adversarial examples in NLP are texts that appear similar to normal text from a human perspective but change the model prediction impacting the model performance. The existence of these adversarial examples raises serious concern regarding both the security and integrity of deep NLP models; thus, to ensure trust, it is crucial to deploy a proper strategy to handle them \cite{amodei2016concrete}. Research work on adversarial attacks can be divided into two groups generation of adversarial \cite{yoo-etal-2020-searching,8424632,kuleshov2018adversarial,wang1909natural} or defense \cite{yuan2019adversarial}.  As research effort to produce adversarial examples has exploded \cite{li-etal-2021-contextualized,ribeiro-etal-2020-beyond,li-etal-2020-bert-attack,garg-ramakrishnan-2020-bae,alzantot-etal-2018-generating,ebrahimi-etal-2018-hotflip,jia-etal-2019-certified,ren-etal-2019-generating,feng-etal-2018-pathologies,li2018textbugger,zang2019word,jin2020bert}  in recent years and become more accessible \cite{morris2020textattack,zeng-etal-2021-openattack}, defending against adversarial samples has received less attention. 

To defend a neural network against adversarial attacks, two main lines of research exist robust training and detection. Robustness techniques involve custom training \cite{yoo-qi-2021-towards-improving,zhou2021defense,pruthi-etal-2019-combating}  to ensure a valid model prediction even when exposed to adversarial examples. The main drawback is to involve an additional training \cite{bao-etal-2021-defending} which also scarifying performance points to ensure robustness \cite{zhou-etal-2019-learning}. Alternatively, the goal of detection is to correctly discriminate an adversarial sample from a normal one without retraining. Although works on detecting adversarial attacks exist in NLP, they primarily focus \textcolor{red}{on learning} on a single attack \cite{le-etal-2021-sweet} or are limited to miss-spelling \cite{pruthi-etal-2019-combating}, making them not usable in practice. To the best of our knowledge, the recent work from \cite{yoo2022detection} is the first to propose a detector that can be applied to various adversarial attack detection. They study the Mahalanobis distance \cite{mahalanobis1936generalized} that has been successfully applied in various out of distribution detection applications \cite{mahalanobis,ren2021simple}. 

%\textbf{Contributions:} In our work, we address the problem of adversarial attack detection and cast it as an anomaly detection problem: adversarial attacks are identified as abnormal observations and we make no assumption about the data distribution. Formally our contributions are threefold:
%\begin{enumerate}[wide, labelwidth=!, labelindent=0pt]
% \item \textbf{A new detector.} We explore the idea of using statistical depth for adversarial attack detection. Statistical depths, originally introduced by \cite{Tukey75} provide a centrality score of a point w.r.t a reference distribution in $\mathbb{R}^d$ with $d>1$. The higher the score, the deeper the point is in the reference distribution. Specifically, our detector (named {\DETECTOR}\footnote{{\DETECTOR} stands for textua\underline{\textbf{L}} \underline{\textbf{A}}dversa\underline{\textbf{R}}ial detecti\underline{\textbf{O}}r Using half\underline{\textbf{S}}pace ma\underline{\textbf{S}}s d\underline{\textbf{E}}pth}) uses the Halspace-mass depth ($D_{HM}$) \cite{chen2015half} which is both robust and can be efficiently computed. Contrarily to the widely used Mahalanobis distance, $D_{HM}$ does not rely on a Gaussian Assumption on the latent space and is also non-differentiable \cite{Xie2019FeatureDF}. Non-differentiability adds a layer of security in the case of total knowledge, as the adversary cannot compute the gradient of the depth.
% \item \textbf{A large benchmark of textual attacks.} To benchmark our method, we develop a new benchmark called {\BENCHMARK} for adver\textbf{\underline{S}}arial a\textbf{\underline{T}}t\textbf{\underline{A}}c\textbf{\underline{K}} b\textbf{\underline{E}}nchmark f\textbf{\underline{O}}r text\textbf{\underline{U}}al da\textbf{\underline{T}}a. To the best of our knowledge, {\BENCHMARK} is the most diverse existing benchmark for textual attack detection. It comprises 9 different attacks performed on 2 different pretrained encoders on 3 different datasets. {\BENCHMARK} will be publicly released in \texttt{DATASETS} to benchmark new detection methods and reduce the computational overhead. 
% \item \textbf{Experimental Contributions \& Code} We demonstrate that {\DETECTOR} is better suited for adversarial detection while having appealing properties (\textit{i.e.,} no hyper-parameter tuning, non-differentiable). In our experimental study, we also highlight and quantify (unreported) factors that induce variations when measuring the detection performance (\textit{i.e.,} dataset choice, selection of clean samples). Lastly, we explore the possibility of building better detectors by exploiting the information in different encoder layers. Our code will be made available on \url{github.com} to ensure reproducibility and accelerate future research; we firmly believe our ideas can be pushed further and provide more robust and reliable NLP classifiers.
%\end{enumerate}


%\section{Background}
%\subsection{Problem Formulation: Attack \& Detection}
%Consider a training dataset denoted by $\mathcal{D} = \{x_i,y_i\}_{i=1}^n$ which is composed of $n$ text $x_i \in \mathcal{X}$ paired together with attribute values $y_i \in \mathcal{Y}\equiv \{1,\dots, |\mathcal{Y}|\}$. In this work, the inputs are first embedded through a multi layer encoder with $L$ layers and learnable parameters $\psi \in \psi$. Denote by $f^\ell_\psi : \mathcal{X} \rightarrow \mathbb{R}^d$ the function which maps the input text to the $\ell$-th layer of the encoder. Note that as we will work on transformer models, the latent space (\textit{i.e.,} the output of a layer) dimension of all layers is the same and denoted by $d$. The dimension of logits, denoted as layer $L+1$ of the encoder is $d^\prime$. We also have access to a pretrained classifier that produces a soft decision over the classes $C_{\psi} : \mathcal{X} \rightarrow [0,1]^{|\mathcal{Y}|}$, with learnt parameters $\psi$.  Given an input $x$, the predicted label $\hat{y}$ is obtained as follows:
%\begin{align*}
%\hat{y} \triangleq \underset{c \in \mathcal{Y}}{\text{arg max}} \; C_{\psi}\left( c|x \right)
% \end{equation} 
% \begin{equation}
%\text{ with } C_{\psi}\left(\cdot|x \right)= \text{softmax} (f_{\psi}^{L+1}(x)). %(\frac{\exp\left( f_{\psi, c}^{L-1}(x; \data)\right)}{\sum _{c'}\exp\left( f_{\psi, c'}^{L-1}(x; \data)\right)},
%\end{align*}

%\textbf{Adversarial Attack} Considering an input $x\in\mathcal{X}$, the problem of adversarial attack generation \cite{ribeiro-etal-2018-semantically,wallace-etal-2019-universal} can be defined as finding an text $x^{\prime}$ such that : 
%\begin{equation}
%\text{max } \text{SIM} \left(x^{\prime}  x \right) \text{~~s.t.~~} \underset{c \in \mathcal{Y}}{\text{arg max}} \; C_{\psi}\left( c|x^{\prime} \right) \neq \underset{c \in \mathcal{Y}}{\text{arg max}} \; C_{\psi}\left( c|x \right),
%\label{eq:adversarial_problem}
%\end{equation}
%where $\text{SIM} : \mathcal{X} \times \mathcal{X} \rightarrow \mathbb{R}^+$ is a function that measures the semantic equivalence between two input texts. Finding a good similarity function for textual data is an active area of research. To quantify the semantic equivalence, previous works \cite{li2018textbugger} rely on embedding similarities such as Word2vect \cite{mikolov2013efficient} of USE \cite{cer-etal-2018-universal} or string based distance \cite{8424632} such as the Leveinshtein distance \cite{levenshtein1965leveinshtein}.

%\textbf{Adversarial Attack Detection} Given an input sentence $x \in \mathcal{X}$, the goal of adversarial attack detection is to build a binary decision rule $d : \mathcal{X} \rightarrow \{0,1\}$ that assigns $1$ to \emph{adversarial samples} created by the malicious attacker and $0$ to \emph{clean samples}. This decision rule relies on a score function $s: \mathcal{X} \rightarrow \mathbb{R}$, and a threshold $\gamma \in \mathbb{R}$ defined as: 
%\begin{equation}
% g(x) = \mathbb{I}{\{s(x) > \gamma\}} = \begin{cases}
%1 \text{ if } s(x) > \gamma, \\
%0\text{ if } s(x) \leq \gamma .\\
%\end{cases} 
%\label{eq:detector}
%\end{equation}


\subsection{Related Works}

\textbf{Adversarial attacks in NLP.} The landscape of available adversarial textual attacks keeps growing, with numerous attacks of different types every year \cite{li-etal-2021-contextualized,ribeiro-etal-2020-beyond,li-etal-2020-bert-attack,garg-ramakrishnan-2020-bae,alzantot-etal-2018-generating,jia-etal-2019-certified,ren-etal-2019-generating,feng-etal-2018-pathologies,li2018textbugger,zang2019word}. Attacks can be broadly grouped according to the perturbation level (\textit{i.e.} character level \cite{ebrahimi-etal-2018-hotflip,pruthi-etal-2019-combating}, word level \cite{jin2020bert}, or sentence level \cite{iyyer-etal-2018-adversarial}) imposed on the input example. Character level attacks often rely on basic operations at the character level, such as substitution, deletion, swap insertion, or repeating. Word level attacks mostly conduct advanced word substitution (\textit{e.g.} using synonyms or semantically equivalent words \cite{miller1995wordnet,miller1990introduction}) and word addition and deletion. At the sentence level, attackers rely on paraphrasing or text generation based on an encoder-decoder structure. Standard toolkits such as \texttt{OpenAttack} \cite{zeng-etal-2021-openattack} or \texttt{Textattack} \cite{morris2020textattack} gather these attacks in a unified framework.


\textbf{Detecting Adversarial Attacks.} Compared to adversarial attack generation, adversarial detection has received drawn much less attention from the NLP community \cite{mozes-etal-2021-frequency}. Detection of adversarial examples has been previously used in the training of classifiers, where it is often considered as a side task \cite{tan-etal-2020-mind,liu2020robust} as the main goal is to achieve robustness. Previous work either supposing access to a specific online generator \cite{dong2021towards,wang2020infobert,yoo-qi-2021-towards-improving} which may not be representative of the variety of existing attacks or makes the unrealistic assumption that adversarial samples are available \cite{xie2022identifying}. Perhaps, a more practical and realistic defense is to rely on perturbation detection without retraining the classifier. In this vein, \cite{mozes-etal-2021-frequency} propose to assess the sentence likelihood based on word frequency, \cite{le-etal-2021-sweet} focused on one type of attack \cite{wallace-etal-2019-universal} while \cite{pruthi-etal-2019-combating} only detect character-level perturbations. In addition to being intrinsically limited \emph{they require adversarial samples for training or validation}. Recent work from \cite{yoo2022detection} is the closest work to us; it relies on the Mahalanobis distance, which has been widely used in Out-of-distribution detection \cite{podolskiy2021revisiting,ren2021simple,kamoi2020mahalanobis}. Different from existing methods, {\DETECTOR} builds on the Halfspace-mass depth that remains overlooked by the Machine Learning community.

%\section{Detecting Adversarial Attacks with {\DETECTOR}}

%\subsection{A brief review of Data Depths}
%\textcolor{red}{envois du lourd guigui}

%\subsection{{\DETECTOR} presentation}
%\textbf{{\DETECTOR} in a nutshell.} Our framework for adversarial attack detection relies on three distinct steps: 
%\begin{enumerate}[wide, labelwidth=!, labelindent=0pt]
%    \item \textbf{Feature Extraction} Recent work on adversarial attack detection on pretrained transformers rely on the last layer of the transformer to compute an anomaly score. Formally, given an input sentence $x$ the associated embedding $z$ is computed through:
%\begin{equation}
% z \triangleq f_\psi^L \left(x\right) \in \mathbb{R}^d.
%\end{equation}
%\item \textbf{Anomaly Score Computation} The second step, rely on a chosen anomalies score and use the Halspace Mass depth. For each class $y \in \mathcal{Y}$ we define $\widetilde{\mathcal{S}}^{L}_{y} \triangleq \{ f_{\psi}^{L}(x_i): x_i \in \mathcal{X} s.t. y_i = y \}$, the set of embeddings of the input in the training set that are associated with label y. Thus, our score function $s_{\DETECTOR}$ boils down to:

%\begin{equation}
% s_{\DETECTOR}(x) \triangleq D_{\mathrm{HM}}\left(z,S_{\hat{y}}\right)
%\end{equation}
%where $D_{\mathrm{HM}}(\cdot,P)$ denotes the halfspace mass depth and $\hat{y}$ denotes the prediction done by the classifier when $x$ is seen as an input.
%\item \textbf{Thresholding} Similar to previous work, the final step consists in using the previous similarity score. If $D\left( F_{PM}(\mathbf{x}), F_{PM}(X_{in}) \right) \leq \delta$, we classify $\mathbf{x}$ as an adversarial attack.
%\end{enumerate}

%\textbf{Efficient Score Computation} Exact computation of $D_{\mathrm{HM}}$ is not possible. To approximate $D_{\mathrm{HM}}$, we rely on a approximation algorithm which in \autoref{}. For each class of $y \in \mathcal{Y}$, we repeat the approximation procedure. Three main parameters are involved $K$ corresponding to the number of direction sampled on the sphere, $n_s$ the sub-sample size which is drawn at each projection step and $\lambda$ which controls the extent of the choice of the hyperplane. These parameter have low sensitivity and we follow and set $K=10000$, $n_s = 32$ and $\lambda = 0.5$. \textcolor{red}{guillaume?}

%\subsection{Link to Mahalanobis based approach}

% another depths of interrest is:
% pas de stocker les matrices de covariance,
% inverser qui
% pbs de conditionnement avec mahanolivs
%The Mahalanobis distance \cite{chandra1936generalised} is a distance between an element in $\mathbb{R}^d$ and a probability distribution having finite expectation and invertible covariance matrix differing from the Euclidean by taking account of correlations. The Mahalanobis distance may define a depth function with an appropriate rescaling as suggested in \cite{Liu92rank}. Precisely, the Mahalanobis depth function is defined as:

%\begin{align*}
%	D_{\mathrm{M}}(x,p_X)= \left( 1+  (x-\mathbb{E}[X])^\top\Sigma^{-1}(x-\mathbb{E}[X])  \right)^{-1},
%\end{align*}
%where $\Sigma^{-1}$ is the precision matrix of the r.v.\ $X$.
%Even though interesting results relying on this notion have been highlighted in \cite{podolskiy2021revisiting}  for OOD detection, this approach is limited as it require to compute $\Sigma^{-1}$ in high dimension, which is the setting of latent representations of transformers. First, only few samples are available  (\textit{e.g.} one sample corresponds to one text in this paper) leading to low-rank matrix $\Sigma$. Therefore, a preliminary projection step is needed in order to invert a covariance matrix computed on projected data. This step leads to a additional computation cost and often a loss of information. Second, inverting $\Sigma$ requires $O(d^3)$ operations and computational burden may arise in high dimension as it is the case for latent representations of transformers. In contrast, the IRW depth does not require to have the first two moments finite neither to compute any covariance matrix making it an attractive choice. 

%The presence of the correlation term in the Mahalanobis definition ensures the affine-invariance of $D_{\mathrm{M}}$ which is crucial in practice since it allows to not take account of the underlying coordinate systems. However, it is non-necessary to have such strong notion of invariance and scale/translation invariance is often sufficient as it is the case for the IRW depth.


%\section{{\BENCHMARK} Presentation}\label{sec:benchmark}
%Textual attack generation can be GPU hungry as some attacks require hundred of queries to corrupt a single sample. Building a benchmark that gathers the result of diverse attacks on different datasets and encoders is of high interest to accelerate and reduce the computational overhead of future research in adversarial attack detection. For gathering the benchmark, we rely on models, dataset and attacks available in \texttt{TextAttack} \cite{morris2020textattack}. In what follow, we describe the experimental choices when building {\BENCHMARK}, discuss our baseline choices and describe our evaluation pipeline.

%\subsection{Benchmark Construction}
%\begin{minipage}{.65\textwidth}
%\textbf{Datasets} For our benchmark, we choose to work on sentiment analysis using SST2 \cite{socher-etal-2013-recursive} and IMDB \cite{maas-etal-2011-learning}) and topic classification relying on ag-news \cite{joachims1996probabilistic}. The choice of these dataset has been motivated by previous work \cite{yoo2022detection}. 
%\\\noindent\textbf{Target Pretrained Classifiers} We rely on the model available on the Transformers' Hub \cite{wolf-etal-2020-transformers}. To ensure that our conclusions are not model specific, we choose to work with classifier based on two types of pretrained encoders: \texttt{BERT} (\texttt{BERT.}) \cite{devlin-etal-2019-bert} and \texttt{ROBERTA} (\texttt{ROB.}) \cite{liu2019roberta}. \autoref{tab:accu} reports the accuracy of the different models on each considered dataset.
%\end{minipage}\quad
%\begin{minipage}{.3\textwidth}
%\resizebox{\textwidth}{!}{\begin{tabular}{ccc}\hline
%   Model  & Dataset & Acc \\\hline
%  \texttt{BERT}   & \texttt{SST2}& \\
%      & \texttt{ag-news}& \\
%       & \texttt{IMDB}&\\
%        \texttt{ROB}   &\texttt{SST2} & \\
%      & \texttt{ag-news}&\\
%       &\texttt{IMDB}& \\\hline
%\end{tabular}}
% \captionof{table}{Classifier accuracy for each considered %dataset}\label{tab:accu}
%\end{minipage}

%\textbf{Adversarial attack} Among the numerous available attacks, we choose to focus on 9 attacks of the 16 methods offered by \texttt{TextAttack}. We tried additional attacks, and they were either too weak to fool the models \cite{ribeiro-etal-2020-beyond,feng-etal-2018-pathologies} or were crashing. \cite{zang-etal-2020-word}. Specifically, we work with  PRUthi (PRU)  \cite{pruthi-etal-2019-combating}, TextBugger (TB) \cite{li2018textbugger}, IGa (IG) \cite{wang2019natural}, DeepWordBug  (DWB) \cite{8424632}, KULeshov (KUL) \cite{kuleshov2018adversarial}, BAE (BAE) \cite{garg-ramakrishnan-2020-bae}, PWW (PWWS) \cite{ren-etal-2019-generating}, TextFooler (TF)\cite{jin2020bert} and TF-adjusted\cite{morris-etal-2020-reevaluating}  (TF-ADF). Further detailed on the attacks are gathered in \autoref{tab:benchmark_considered_attacks}. \autoref{fig:benchmark_sucess} displays the attack success rate per classifier on the different datasets.  
%\\\noindent\textit{Takeaways.} Interestingly, attack efficiency only marginally depends on the pre-trained encoder choice. In contrast, we observe a strong dependency on the training set (variation of over 0.1 efficiency points). It is worth noting that TF and KUL are the most efficient attacks. Interestingly, attack efficiency only marginally depends on the pre-trained encoder choice.
% \begin{figure}[!ht]
% \centering
% \centering
% \includegraphics[width=\textwidth]{efficiency_ratio.pdf}
% \caption{Efficiency of the choosen attacks. Both checklist and %input-reduction were tried but discarded due to low. It is worth %noting that IG fails on IMDB.}
% \label{fig:benchmark_sucess}
% \end{figure}
%\\\noindent\textbf{Adversarial and Clean sample selection} Several ways of selecting both adversarial and clean samples exist. In our setting, we select the one that changes the classifier decision among correctly classified samples as adversarial text. As we will see in \autoref{sec:expe}, a key for evaluating detection performance is to select the clean samples. Following \cite{yoo2022detection}, we sample clean samples from a disjoint set of the clean samples used for adversarial attack detection. For all our experiments, we ensure a balanced ratio of clean and adversarial samples.


%\subsection{Baselines} 
%\textbf{Baseline Detector} We compare the the performances of {\DETECTOR} we presented with a baseline based on language model (LM) scores and following \cite{mahalanobis,yoo2022detection}, we also rely on a Mahalanobis-based detector.
%\begin{enumerate}[wide, labelwidth=!, labelindent=0pt]
%    \item \textbf{Language Model Scores}.The basic idea of using a LM for adversarial detection is to rely on a pretrained LM and check how likely the input instance is. Formally, the associated score function as defined in \autoref{eq:detector} is $s_{LM}(x) = \sum_{i=1}^{|x|} - \log p_{\psi}(x_i| x_{i-1}, \cdots, x_1)$ where $x_i$ are the token composing the input text $x$ and the log probability are given by the output of a pretrained \texttt{GPT2} \cite{NEURIPS2020_1457c0d6}. 
% \item  \textbf{Mahalanobis-based detector}. We follow \cite{mahalanobis,yoo2022detection} which rely on a class conditioned Mahalanobis distance. Formally following our notations  $s_{M}(x) \triangleq \left(f_\psi^L(x) - \mu_{\hat{y}}\right)^T \Sigma_{\hat{y}}  \left(f_\psi^L(x) - \mu_{\hat{y}}\right) $ where $\mu_{\hat{y}}$ the empirical mean for the logits of class $\hat{y}$ and $\Sigma_{\hat{y}}$ represents the empirical covariance.
% \item \textbf{Feature Extraction} Both the Mahanalobis and $D_{HM}$ scores are computed based on the layer outputs. To better understand the impact of different features, we follow previous work \cite{podolskiy2021revisiting,yoo2022detection} and rely on the penultimate layer (layer $L$) of the encoder or the logits (layer $L+1$).
%\end{enumerate}

%\begin{remark}
%Although pretrained models relies on several layer and the idea of using information available in multiple layers seems appealing, this idea appears to be unfruitful (see \autoref{sec:all_info}).
%\end{remark}


%\subsection{Evaluation}
%The adversarial attack detection problem can be seen as a classification problem. We rely on the {\it false alarm rate}, \textit{i.e.} the proportion of samples that are miss-classified as \emph{adversarial sample} while they are \emph{clean}. Similarly, we use the {\it true detection rate}, \textit{i.e.,} the proportion of samples that are rightfully predicted \emph{adversarial sample}. Although many different quantities can be defined for our setting, we choose to focus on three different metrics that assess the quality of our method. 
%\begin{enumerate}[wide, labelwidth=!, labelindent=0pt]
 %   \item \textbf{Area Under the Receiver Operating Characteristic curve \cite{bradley1997use} ({\AUROC}).} It is the area under the ROC curve which consider the true detection rates against the false alarm rates. From elementary computations, the {\AUROC} can be linked to the probability that an clean example has higher score than an adversarial sample.
 % \item \textbf{Area Under the Precision-Recall curve (\texttt{AUPR}) \cite{davis2006relationship}}. It is the area under the precision-recall curve which is more relevant to imbalanced situations. It plots the recall (true detection rate) against the precision (actual proportion of \emph{adversarial sample} amongst the predicted \emph{adversarial sample}).
 %\item \textbf{True Negative Rate at 95\% True Positive Rate (\texttt{TNR@TPR-95\%} (\%))}. In practical situation, one build a strong detector. Thus, given a detection rate $r$, this incites to fix a threshold $\delta_r$ such that the corresponding TPR equals $r$. Following \cite{}, we set $r = 0.90$.
%\end{enumerate}



\subsection{Overall Results}\label{ssec:overall_results}
We report in \autoref{tab:all_average_main} the aggregated performance over the different datasets, the different seeds , and the different attacks.
\\\noindent \textbf{$D_{\mathrm{HM}}$ achieve the best overall results.} It is worth noting that detection methods better discriminate adversarial attacks on \texttt{ROB.} than \texttt{BERT}. It also consistently improves when using $D_{\mathrm{HM}}$ over $D_{\mathrm{M}}$, which experimentally validates our choice. This conclusion holds on both \texttt{ROB.} and \texttt{BERT}, corresponding to over $540$ experimental configurations. Similar to previous work \cite{yoo2022detection}, the detector built on \texttt{GPT2} under-performs $D_{\mathrm{M}}$. For all methods we observe that threshold-free metrics (\textit{e.g.} {\AUROC}, {\AUPRIN} and {\AUPROUT}) threshold-based metrics (\textit{e.g.} {\FPR}). 
\\\noindent \textbf{Importance of feature selection for adversarial detectors.} Both $D_{\mathrm{HM}}$ and $D_{\mathrm{M}}$ are highly sensitive to the layer's choice. For $D_{\mathrm{M}}$, using the logits is better than the penultimate layer, while for $D_{HM}$, the converse works better. Although the AUROC presents a slight variation when using $f_\psi^{L+1}$ instead of $f_\psi^{L}$, it induces a variation of over 10 {\FPR} points.

Overall, it is worth noting the best detectors (\textit{i.e.} using $D_{\mathrm{HM}}$) although being state-of-the art on tested configuration, achieve an {\FPR} which remains moderate. The best detector achieves an averaged error of $17.9\%$ which is far from the accuracy achieved on the main task (over 90\% on all datasets). 


%\input{total_average}
% tableau en gras
\begin{figure}
\centering
\begin{subfigure}[b]{\textwidth}
 \centering
 \includegraphics[width=\textwidth]{results_all_images/auroc_attack_nogpt.pdf}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
 \centering
 \includegraphics[width=\textwidth]{results_all_images/fpr_attack_nogpt.pdf}
\end{subfigure}
\caption{Performance in terms of {\AUROC} (up) and {\FPR} (down)  of $D_{\mathrm{M}}$ and $D_{\mathrm{HM}}$ for the different attacks across the three considered datasets. \autoref{fig:all_results_per_attack_appendix} reports the results of \texttt{GPT2}, which were omitted for clarity purposes. }
\label{fig:all_plots_per_model}
\end{figure}

\subsection{Identifying Key Detection Factors}
To better understand the performance of our methods w.r.t different attacks and different datasets, we report in \autoref{fig:all_plots_per_model} the performance in terms of {\AUROC} and {\FPR} per attack. 
\\\noindent \textbf{Detectors and models are not robust to dataset change.} The detection task is more challenging for SST-2 than for ag-news and IMDB, with a significant drop in performance  (\textit{e.g.} over 15 absolute points for BAE). On SST-2, $D_{\mathrm{HM}}$ achieves a significant gain over $D_{\mathrm{M}}$ both for the {\AUROC} and {\FPR}. 
\\\noindent \textbf{Detectors do not detect uniformly well all the different attacks.} This phenomenon is pronounced on SST2 while beeing present for both ag-news and IMDB. For example on SST2, {\FPR} varies from less than 10 (a strong detection performance) for TF-ADJ to over 70 (a poor performance) for PRU. 
\\\noindent \textbf{The choice of clean samples largely affect the detection performance measure.} \autoref{fig:all_plots_per_model} displays several tries with different seed. As mentioned in \autoref{sec:benchmark}, different seeds correspond to different choice of clean samples. On all datasets we observe that when measuring the algorithm performance different negative samples will lead different results (\textit{e.g.} {\FPR} on IMDB varies of over 30 points on KUL and PRU across different seeds).



\begin{figure}
\centering
\begin{subfigure}[b]{0.32\textwidth}
 \centering
 \includegraphics[width=\textwidth]{tradeoffs/trade_off_auroc_fpr_attakcs.pdf}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
 \centering
 \includegraphics[width=\textwidth]{tradeoffs/trade_off_auprin_fpr_attakcs.pdf}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
 \centering
 \includegraphics[width=\textwidth]{tradeoffs/trade_off_auprout_fpr_attakcs.pdf}
\end{subfigure}
\caption{Empirical study of the metric relationship for the three considered detection methods.}
\label{fig:all_tradeoff_main}
\end{figure}
\subsection{All the metrics matter}
\textbf{Setup} In this experiment we study the relationship between the different metrics. From \autoref{tab:all_average_main}, we see that threshold free metrics (\textit{i.e} {\AUROC}, {\AUPRIN} and {\AUPROUT}) exhibit lower variance than threshold based metrics such as {\FPR}. The {\FPR} measures the percentage of natural samples detected as adversarial when $90\%$ of the attacked samples are detected. Therefore, the lower is, the better. 
\\\noindent \textbf{Takeaways} From \autoref{fig:all_tradeoff_main}, we see that a large {\AUROC}, {\AUPRIN} and {\AUPROUT} do necessarily correspond a low {\FPR}. This suggests that the detectors also detect natural samples as adversarial when it detect at least 90$\%$ of adversarial samples. Additionally, a small variation of {\AUROC}, {\AUPRIN} and {\AUPROUT} can lead to a high change in {\FPR}. Since a high {\AUROC}, {\AUPRIN} and {\AUPROUT} do not imply a low {\FPR} it is crucial to compare the detectors using both metrics. 
\subsection{What Performance to Expect From {\DETECTOR}?}
\begin{minipage}{.4\textwidth}
    \includegraphics[width=\textwidth]{practical_detector/error_detector.pdf}
    \captionof{figure}{Detection error on {\BENCHMARK}}\label{fig:crafting_a_detector}
\end{minipage}\quad
\begin{minipage}{.55\textwidth}
\textbf{Setup} \autoref{fig:crafting_a_detector} reports the error probability per attack for {\DETECTOR} and the considered baselines. 
\\\noindent \textbf{Efficient attacks are easier to detect.} We observe that on the three most efficient attacks, according to  \autoref{fig:benchmark_sucess} (\textit{i.e.,} TF, PWWS and KUL), {\DETECTOR} is more significantly more effective than $D_{\mathrm{M}}$ and \texttt{GPT2}. 
\\\noindent \textbf{Different detection methods capture different phenomena are better suited for detecting different attack types.}  Although {\DETECTOR} achieves the best results overall, \texttt{GPT2}, which relies on perplexity solely, achieves competitive results with {\DETECTOR} and outperforms $D_{\mathrm{M}}$ on several attacks (\textit{i.e.,} DWB, IG). This suggests that stronger detectors could be achieve by combining different types of scores function.

\end{minipage}
\section{Future Research Directions \& Conclusions}

\subsection{Measuring Information Available in the Encoder Layers}\label{sec:all_info}
A promising research direction to improve the detector is to develop an unsupervised strategy for combining multiple-layer representations of the pre-trained encoders. Combining, multiple layers of a pre-trained encoder has been shown to be a successful idea in the case of image \cite{gomes2022igeood,sastry2020detecting}, but never shown to be useful in text. 
\\\noindent \textbf{Setup} In this experiment, we aim to quantify the power of each layer to discriminate between clean and adversarial samples. To measure this discriminative ability, we rely on Wasserstein distance ($\mathcal{W}_1$) (see e.g. \cite{Peyre}). Given two empirical distribution, $\mathcal{W}_1$ finds the best possible transfer between them while minimizing the transportation cost defined by the Euclidean distance. \autoref{fig:impossibility} reports the transportation cost between the empirical distribution, obtained by the representation of each layer, of clean samples ($\mu_{clean}$), adversarial samples ($\mu_{adv}$) and the training samples ($\mu_{train}$). 
\\\noindent\textbf{Takeaways} \textcolor{red}{discuter des plots finales}
\begin{figure}[!ht]
 \centering
 \subfloat[\centering $\mathcal{W}_1\left(\mu_{train},\mu_{adv}\right)$ ]{{\includegraphics[width=4cm]{layerwise/results_layers_train_adv.pdf} }}%
 \qquad
 \subfloat[\centering $\mathcal{W}_1\left(\mu_{train},\mu_{clean}\right)$  ]{{\includegraphics[width=4cm]{layerwise/results_layers_train_clean.pdf} }}%
 \qquad
 \subfloat[\centering $\mathcal{W}_1\left(\mu_{adv},\mu_{clean}\right)$ ]{{\includegraphics[width=4cm]{layerwise/results_layers_clean_adv.pdf} }}%
 \caption{2 Figures side by side}%
 \label{fig:impossibility}%
\end{figure}


\subsection{Conclusions}




\clearpage
\fi

==> contributions.tex <==
% Nouveau Score
% Faire un trucs
% Etude de la pertinence des layers 

% A l'interieur des layers couts de transport.


==> explore_attack.tex <==
\begin{tabular}{lllrr} \hline
\toprule                  &      &            &  ratio &      query \\   
model & ds & attack &        &            \\  \hline 
\midrule 
bert-base-uncased & ag-news & bae &  0.245 &    110.339 \\   
&      & checklist &  0.070 &     25.323 \\       
&      & clare &  0.952 &   8139.813 \\  
&      & deepwordbug &  0.640 &     88.468 \\ 
&      & iga &  0.578 &   3374.795 \\        
&      & input-reduction &  1.000 &        NaN \\             
&      & kuleshov &  0.828 &   1137.360 \\   
&      & pruthi &  0.155 &    734.253 \\       
&      & pwws &  0.593 &    325.982 \\    
&      & textbugger &  0.593 &    139.048 \\  
& imdb & bae &  0.661 &    406.026 \\        
&      & checklist &  0.144 &    254.277 \\
&      & clare &  1.000 &  23819.739 \\     
&      & deepwordbug &  0.792 &    279.784 \\  
&      & input-reduction &  1.000 &        NaN \\   
&      & kuleshov &  1.000 &   8446.076 \\   
&      & pruthi &  0.332 &   3952.905 \\      
&      & pwws &  0.997 &   1462.160 \\       
&      & textbugger &  0.934 &    461.961 \\  
& sst2 & bae &  0.675 &     67.484 \\        
&      & checklist &  0.078 &      3.500 \\    
&      & clare &  0.997 &   1545.301 \\   
&      & deepwordbug &  0.826 &     31.651 \\   
&      & iga &  0.892 &    733.101 \\ 
&      & input-reduction &  1.000 &        NaN \\       
&      & kuleshov &  0.929 &    218.743 \\        
&      & pruthi &  0.408 &    309.107 \\    
&      & pwws &  0.876 &    148.328 \\      
&      & textbugger &  0.783 &     51.412 \\ 
roberta-base & ag-news & bae &  0.289 &    112.349 \\  
&      & checklist &  0.073 &     30.446 \\        
&      & clare &  0.934 &   8483.163 \\   
&      & deepwordbug &  0.609 &     88.639 \\  
&      & iga &  0.632 &   3224.543 \\  
&      & input-reduction &  1.000 &        NaN \\  
&      & kuleshov &  0.847 &   1100.484 \\   
`&      & pruthi &  0.166 &    727.355 \\    
&      & pwws &  0.674 &    324.123 \\                  &      & textbugger &  0.593 &    142.516 \\         
& imdb & bae &  0.703 &    399.287 \\  
&      & checklist &  0.077 &    438.966 \\                  &      & clare &  1.000 &  23589.572 \\                  &      & deepwordbug &  0.725 &    283.390 \\    
&      & input-reduction &  1.000 &        NaN \\                  &      & kuleshov &  1.000 &   6706.383 \\         
&      & pruthi &  0.158 &   4218.255 \\      
&      & pwws &  0.994 &   1532.497 \\                  &      & textbugger &  0.939 &    523.026 \\   
& sst2 & bae &  0.669 &     69.245 \\     
&      & checklist &  0.060 &        NaN \\                  &      & clare &  0.997 &   1545.237 \\    
&      & deepwordbug &  0.829 &     34.592 \\  
&      & iga &  0.867 &    774.523 \\                  &      & input-reduction &  1.000 &        NaN \\  
&      & kuleshov &  0.922 &    236.900 \\   
&      & pruthi &  0.360 &    285.050 \\    
&      & pwws &  0.856 &    149.677 \\      
&      & textbugger &  0.737 &     55.513 \\ 
\bottomrule     
\end{tabular}     '

==> per_attack.tex <==
\begin{table}[]
 \caption{Which attacks are the hardest to detect? }
    \label{tab:attack_difficulty}
    \centering
\begin{tabular}{cccccccc}  \toprule     
&                    &        &  {\AUROC} &  {\FPR} &{\AUPRIN} &{\AUPROUT}&{\ERR} \\
\midrule         BAE & empirical & $f_\theta^{L+1}$ &   \result{87.7} {       10.5 }&\result{  26.6} {     22.8 }&\result{     85.7} {         13.7} &\result{      86.6} {           9.5 }&\result{   18.2} {       11.4 }\\ 
& GPT2 &$f_\theta^L$                        &   \result{68.8} {        4.4 }&\result{  72.3} {      6.2 }&\result{     67.9} {          4.3} &\result{      66.9} {           4.8 }&\result{   41.1} {        3.1 }\\ 
& halfspace\_mass\_unn &$f_\theta^L$       &   \result{91.0} {        7.5 }&\result{  22.5} {     19.8 }&\result{     91.0} {          9.0} &\result{      89.4} {           6.8 }&\result{   16.2} {        9.9 }\\   
DWB & empirical & $f_\theta^{L+1}$                  &   \result{90.1} {        6.2 }&\result{  41.7} {     19.3 }&\result{     88.2} {          9.0} &\result{      88.5} {           6.4 }&\result{   23.3} {        9.6 }\\ 
& GPT2 &$f_\theta^L$                        &   \result{87.0} {        6.3 }&\result{  35.2} {     15.9 }&\result{     85.9} {          6.6} &\result{      87.4} {           6.2 }&\result{   22.4} {        7.9 }\\        
& halfspace\_mass\_unn &$f_\theta^L$       &   \result{92.7} {        3.3 }&\result{  43.1} {     16.2 }&\result{     93.8} {          3.2} &\result{      90.3} {           4.0 }&\result{   23.9} {        8.1 }\\ 
IG & empirical & $f_\theta^{L+1}$                   &   \result{89.3} {        6.7 }&\result{  49.5} {     17.1 }&\result{     87.1} {         10.0} &\result{      87.6} {           6.9 }&\result{   27.0} {        8.6 }\\          
& GPT2 &$f_\theta^L$                        &   \result{81.6} {        5.2 }&\result{  52.2} {     15.9 }&\result{     81.2} {          5.0} &\result{      79.7} {           6.9 }&\result{   30.9} {        8.0 }\\      
& halfspace\_mass\_unn &$f_\theta^L$       &   \result{91.3} {        1.7 }&\result{  54.4} {     14.0 }&\result{     92.8} {          1.8} &\result{      87.9} {           2.7 }&\result{   29.4} {        6.9 }\\ 
KUL & empirical & $f_\theta^{L+1}$                  &   \result{90.8} {        6.3 }&\result{  40.6} {     19.4 }&\result{     89.5} {          9.3} &\result{      89.6} {           6.5 }&\result{   22.4} {        9.8 }\\    
& GPT2 &$f_\theta^L$                        &   \result{73.9} {        7.7 }&\result{  65.5} {     15.0 }&\result{     74.0} {          6.8} &\result{      72.8} {           8.8 }&\result{   37.0} {        6.8 }\\     
& halfspace\_mass\_unn &$f_\theta^L$       &   \result{93.0} {        3.5 }&\result{  41.7} {     19.4 }&\result{     93.8} {          3.5} &\result{      91.4} {           4.5 }&\result{   22.9} {       10.1 }\\ 
PRU & empirical & $f_\theta^{L+1}$                  &   \result{81.4} {       10.1 }&\result{  62.5} {     17.6 }&\result{     77.8} {         13.4} &\result{      80.9} {           9.1 }&\result{   33.4} {        8.7 }\\      
& GPT2 &$f_\theta^L$                        &   \result{68.2} {        8.4 }&\result{  72.8} {      9.9 }&\result{     69.0} {          8.1} &\result{      66.8} {           7.2 }&\result{   41.0} {        4.7 }\\         
& halfspace\_mass\_unn &$f_\theta^L$       &   \result{87.4} {        6.0 }&\result{  62.0} {     18.7 }&\result{     89.1} {          6.0} &\result{      84.0} {           6.9 }&\result{   33.2} {        9.4 }\\ 
PWWS & empirical & $f_\theta^{L+1}$                 &   \result{89.1} {        7.4 }&\result{  27.0} {     18.7 }&\result{     87.6} {         10.2} &\result{      87.1} {           7.3 }&\result{   18.4} {        9.3 }\\      
& GPT2 &$f_\theta^L$                        &   \result{78.9} {        7.9 }&\result{  52.3} {     18.0 }&\result{     77.6} {          8.1} &\result{      78.7} {           9.1 }&\result{   31.1} {        9.0 }\\         
& halfspace\_mass\_unn  &$f_\theta^L$      &   \result{92.1} {        3.6 }&\result{  24.6} {     14.2 }&\result{     93.2} {          3.9} &\result{      89.0} {           4.0 }&\result{   17.3} {        7.1 }\\  
TB & empirical & $f_\theta^{L+1}$                   &   \result{93.6} {        4.2 }&\result{  29.7} {     17.5 }&\result{     92.8} {          6.1} &\result{      91.7} {           4.6 }&\result{   17.2} {        8.7 }\\         
& GPT2 &$f_\theta^L$                        &   \result{84.3} {        5.8 }&\result{  43.3} {     18.5 }&\result{     83.2} {          5.4} &\result{      83.9} {           7.9 }&\result{   26.5} {        9.2 }\\         
& halfspace\_mass\_unn &$f_\theta^L$       &   \result{95.1} {        2.3 }&\result{  29.6} {     17.2 }&\result{     96.0} {          2.0} &\result{      93.1} {           3.4 }&\result{   17.2} {        8.6 }\\ 
TF & empirical & $f_\theta^{L+1}$                   &   \result{91.9} {        6.5 }&\result{  16.3} {     15.7 }&\result{     90.1} {          9.9} &\result{      90.7} {           6.1 }&\result{   13.1} {        7.8 }\\         
& GPT2 &$f_\theta^L$                        &   \result{80.8} {        7.7 }&\result{  48.1} {     18.2 }&\result{     79.2} {          7.7} &\result{      80.9} {           9.0 }&\result{   29.0} {        9.1 }\\        
& halfspace\_mass\_unn  &$f_\theta^L$      &   \result{93.8} {        3.5 }&\result{  16.3} {     11.9 }&\result{     94.4} {          4.1} &\result{      92.0} {           3.8 }&\result{   13.1} {        5.9 }\\ 
TF-ADJ & empirical & $f_\theta^{L+1}$               &   \result{95.8} {        2.5 }&\result{   9.1} {     13.0 }&\result{     96.8} {          1.7} &\result{      93.9} {           3.9 }&\result{    8.8} {        6.4 }\\         
& GPT2 &$f_\theta^L$                        &   \result{70.1} {        5.2 }&\result{  71.5} {      9.7 }&\result{     70.8} {          5.0} &\result{      68.4} {           6.8 }&\result{   40.0} {        4.7 }\\        
& halfspace\_mass\_unn      &$f_\theta^L$  &   \result{96.9} {        2.4 }&\result{   9.2} {     13.8 }&\result{     97.7} {          1.5} &\result{      95.1} {           4.6 }&\result{    8.8} {        6.9 }\\  

\end{tabular}  

\end{table}

==> total_average.tex <==
\begin{table}[]
    \centering
 \caption{Aggregated performance over both datasets and attacks. Each results aggregates in 270 measurements (10 seeds $\times$ 3 datasets $\times$ 9 attacks.)}\label{tab:all_average}
\begin{tabular}{cccccccc}  \toprule     
&                    &        &  {\AUROC} &  {\FPR} &{\AUPRIN} &{\AUPROUT}&{\ERR} \\
\midrule  \texttt{BERT}  & $D_M$ & $f_\theta^L$ &   \result{88.8} {        6.3} & \result{ 49.7} {     25.4} &     \result{90.9 }{          6.0} & \result{     84.5} {           8.2 }&\result{   28.4} {       12.0} \\  
&                    & $f_\theta^{L+1}$         &   \result{90.1} {        7.8} & \result{ 32.3} {     23.9} &     \result{88.6 }{         10.4} & \result{     88.5} {           7.6 }&\result{   19.7} {       11.3} \\ 
& $GPT2$ & $f_\theta^L$                        &   \result{76.1} {        9.1} & \result{ 58.4} {     19.1} &     \result{75.4 }{          8.7} & \result{     75.3} {          10.2 }&\result{   34.0} {        9.5} \\   
& $D_{HM}$ & $f_\theta^L$                       &   \textbf{\result{92.0} {        5.0}} & \textbf{\result{ 32.1} {     24.1}} &     \textbf{\result{93.3 }{          4.8}} &\textbf{ \result{     89.4} {           5.8 }}&\textbf{\result{   19.5} {       11.2}} \\ % 36.1 21.5
&                    & $f_\theta^{L+1}$         &   \result{91.9} {        5.1} & \result{ 35.8} {     23.2} &     \result{92.4 }{          5.7} & \result{     90.0} {           5.6 }&\result{   21.4} {       10.9} \\ \hline
\texttt{ROB} & $D_M$ & $f_\theta^L$             &   \result{89.9} {        5.5} & \result{ 44.1} {     22.9} &     \result{91.9 }{          5.1} & \result{     86.1} {           7.2 }&\result{   25.5} {       10.9} \\  
&                    & $f_\theta^{L+1}$         &   \result{90.0} {        8.3} & \result{ 31.9} {     23.6} &     \result{88.5 }{         11.5} & \result{     88.7} {           7.8 }&\result{   19.5} {       11.3} \\ 
& $GPT2$ & $f_\theta^L$                        &   \result{77.7} {        9.7} & \result{ 56.0} {     20.4} &     \result{77.2 }{          9.1} & \result{     76.8} {          10.7 }&\result{   32.6} {        9.9} \\       
& $D_{HM}$ & $f_\theta^L$                       &   \textbf{\result{93.4} {        4.6}} & \textbf{\result{ 29.0} {     21.7}} &     \textbf{\result{93.9 }{          5.4}} & \textbf{\result{     91.3} {           5.3 }}&\textbf{\result{   17.9} {       10.3}} \\
&                    & $f_\theta^{L+1}$         &   \result{92.8} {        5.1} & \result{ 32.1} {     23.5} &     \result{93.3 }{          5.9} & \result{     90.9} {           5.9 }&\result{   19.4} {       11.3} \\   
\bottomrule  
\end{tabular} 
\end{table}
